Design and Evaluation of Personalized Free Trials

Free trial promotions, where users are given a limited time to try the product for free, are a commonly used customer acquisition strategy in the Software as a Service (SaaS) industry. We examine how trial length affect users' responsiveness, and seek to quantify the gains from personalizing the length of the free trial promotions. Our data come from a large-scale field experiment conducted by a leading SaaS firm, where new users were randomly assigned to 7, 14, or 30 days of free trial. First, we show that the 7-day trial to all consumers is the best uniform policy, with a 5.59% increase in subscriptions. Next, we develop a three-pronged framework for personalized policy design and evaluation. Using our framework, we develop seven personalized targeting policies based on linear regression, lasso, CART, random forest, XGBoost, causal tree, and causal forest, and evaluate their performances using the Inverse Propensity Score (IPS) estimator. We find that the personalized policy based on lasso performs the best, followed by the one based on XGBoost. In contrast, policies based on causal tree and causal forest perform poorly. We then link a method's effectiveness in designing policy with its ability to personalize the treatment sufficiently without over-fitting (i.e., capture spurious heterogeneity). Next, we segment consumers based on their optimal trial length and derive some substantive insights on the drivers of user behavior in this context. Finally, we show that policies designed to maximize short-run conversions also perform well on long-run outcomes such as consumer loyalty and profitability.

==> Free Trial/Figures/AllMethodsCDFComparison.tex <==
\begin{figure}[!htbp]
    \centering

    \includegraphics[scale = 0.26]{Figures/AllMethodsCDFComparison730_Test.png}
    CDF of $\mathbf{\tau_{7, 30}}$\par\medskip
    
    \includegraphics[scale = 0.26]{Figures/AllMethodsCDFComparison1430_Test.png}
    CDF of $\mathbf{\tau_{14, 30}}$\par\medskip
    
    \includegraphics[scale = 0.26]{Figures/AllMethodsCDFComparison714_Test.png}
    CDF of $\mathbf{\tau_{7, 14}}$\par\medskip
    
    \caption{\label{figure:cdf_comparison_all} 
    The CDF of estimated CATEs from using different methods (for test data).} 
\end{figure}

==> Free Trial/Tables/causal-tree-forest.tex <==
\begin{figure}[t]
  \begin{subfigure}[b]{0.4\textwidth}
    \includegraphics[width=\textwidth]{Figures/tree.PNG}
    \caption{A causal tree}
    \label{figure:causaltreeforest}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.5\textwidth}
    \includegraphics[width=\textwidth]{Figures/forest.PNG}
    \caption{A causal forest}
    \label{fig:f2}
  \end{subfigure}
  \caption{In order to estimate the treatment effect for an observation (the blue dot) in the causal tree algorithm, we use the outcome of the observations that get the treatment (the green dots) and observations that do not get the treatment (the red dots). In the causal forest algorithm, we generate thousands of such trees, and average their results for each observation. Please note that because of the randomness in sub sampling, each tree can be different, and each observation might end up in a partition with different observations.}
\end{figure}

==> Free Trial/Tables/indirect_method_mse.tex <==
\begin{table}[t]
\centering
\footnotesize

\begin{tabular}{l|cc}
\toprule
\multirow{2}{*}{\textbf{Method}} & 
\multicolumn{2}{c}{\textbf{Mean Squared Error}}\\
 & Training Set & Test Set
\\
\hline\hline

 Linear Regression &    0.0932 &    0.0933 \\
             Lasso &    0.0933 &    0.0933 \\
              CART &    0.0916 &    0.0920 \\
     Random Forest &    0.0904 &    0.0915 \\
           XGBoost &    0.0905 &    0.0911 \\

\bottomrule
\end{tabular}
\caption{\label{table:predictive-perf} Comparison of the predictive performance of the five outcome estimation methods. The MSE for any method are calculated as $\frac{\sum_{i = 1}^N(\hat{y}_i-y_i)^2}{N}$, where $\hat{y}_i$ is the prediction of $y_i$ and $N$ is the number of data-points in the data-set being considered.}
\end{table}

==> Free Trial/Tables/overfit_test_2.tex <==
\begin{table}[t]
\centering
\footnotesize
\begin{tabular}{ccc}
\toprule
\textbf{Optimal Trial Length} &
\textbf{ Actual Trial Length}  &   
\textbf{ Subscription Rate} \\

\hline\hline
\multirow{3}{*}{7 Days} & 7 Days &  \textbf{14.3}    \\
 & 14 Days &   13.5   \\
 & 30 Days &   13.3   \\
\midrule
\multirow{3}{*}{14 Days} & 7 Days&  18.3      \\
 & 14 Days &   \textbf{18.8}   \\
& 30 Days &  17.5  \\
\midrule
\multirow{3}{*}{30 Days} & 7 Days&  12.5      \\
 & 14 Days &   12.6   \\
& 30 Days &  \textbf{13.8}  \\

\bottomrule
\end{tabular}
\caption{\label{table:overfit_test_2} Comparison of the predicted subscription rate in the optimal policy that is made using profit valuation hyper-parameter optimization. \hema{With $\%85$ confidence interval the difference average subscription rate in the 30-days optimal case is positive.}}
\end{table}

==> Free Trial/Tables/rev_ate.tex <==
\begin{table}[t]
\centering
\footnotesize
\begin{tabular}{l|cc}
\toprule
\textbf{Treatment} &  \textbf{Revenue difference} &  \textbf{t-statistics}\\
\hline\hline
7 days &  16.53 & 2.36\\
14 days  & 14.69 & 2.10 \\ \bottomrule
\end{tabular}
\caption{\label{table:average_rev} Average effect of the 7- and 14-day treatments on revenues per subscribed user); compared to the control condition of 30-day free-trial.}
\end{table}

==> Free Trial/Tables/time_to_sub.tex <==
\begin{table}[t]
\centering
\footnotesize
\begin{tabular}{l|c}
\toprule
\textbf{Trial Length} &   \textbf{Average difference between initial trial start and subscription}\\
\hline\hline
\textbf{7 days} & 120.9\\
\textbf{14 days} & 128.8\\
\textbf{30 days} & 143.7\\
\bottomrule
\end{tabular}
\caption{\small\label{table:time_to_sub} The average number of days between initial trial start and subscription across users with different trial lengths.}
\end{table}

==> Tables/causal-tree-forest.tex <==
\begin{figure}[t]
  \begin{subfigure}[b]{0.4\textwidth}
    \includegraphics[width=\textwidth]{Figures/tree.PNG}
    \caption{A causal tree}
    \label{figure:causaltreeforest}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.5\textwidth}
    \includegraphics[width=\textwidth]{Figures/forest.PNG}
    \caption{A causal forest}
    \label{fig:f2}
  \end{subfigure}
  \caption{In order to estimate the treatment effect for an observation (the blue dot) in the causal tree algorithm, we use the outcome of the observations that get the treatment (the green dots) and observations that do not get the treatment (the red dots). In the causal forest algorithm, we generate thousands of such trees, and average their results for each observation. Please note that because of the randomness in sub sampling, each tree can be different, and each observation might end up in a partition with different observations.}
\end{figure}

==> Tables/overfit_test_2.tex <==
\begin{table}[t]
\centering
\footnotesize
\begin{tabular}{ccc}
\toprule
\textbf{Optimal Trial Length} &
\textbf{ Actual Trial Length}  &   
\textbf{ Subscription Rate} \\

\hline\hline
\multirow{3}{*}{7 Days} & 7 Days &  \textbf{14.3}    \\
 & 14 Days &   13.5   \\
 & 30 Days &   13.3   \\
\midrule
\multirow{3}{*}{14 Days} & 7 Days&  18.3      \\
 & 14 Days &   \textbf{18.8}   \\
& 30 Days &  17.5  \\
\midrule
\multirow{3}{*}{30 Days} & 7 Days&  12.5      \\
 & 14 Days &   12.6   \\
& 30 Days &  \textbf{13.8}  \\

\bottomrule
\end{tabular}
\caption{\label{table:overfit_test_2} Comparison of the predicted subscription rate in the optimal policy that is made using profit valuation hyper-parameter optimization. \hema{With $\%85$ confidence interval the difference average subscription rate in the 30-days optimal case is positive.}}
\end{table}

==> Tables/rev_ate.tex <==
\begin{table}[t]
\centering
\footnotesize
\begin{tabular}{l|cc}
\toprule
\textbf{Treatment} &  \textbf{Revenue difference} &  \textbf{t-statistics}\\
\hline\hline
7 days &  16.53 & 2.36\\
14 days  & 14.69 & 2.10 \\ \bottomrule
\end{tabular}
\caption{\label{table:average_rev} Average effect of the 7- and 14-day treatments on revenues per subscribed user); compared to the control condition of 30-day free-trial.}
\end{table}

==> Tables/time_to_sub.tex <==
\begin{table}[t]
\centering
\footnotesize
\begin{tabular}{l|c}
\toprule
\textbf{Trial Length} &   \textbf{Average difference between initial trial start and subscription}\\
\hline\hline
\textbf{7 days} & 120.9\\
\textbf{14 days} & 128.8\\
\textbf{30 days} & 143.7\\
\bottomrule
\end{tabular}
\caption{\small\label{table:time_to_sub} The average number of days between initial trial start and subscription across users with different trial lengths.}
\end{table}
